A data-centric weak supervised learning for highway traffic incident detection

Using the data from loop detector sensors for near-real-time detection of traffic incidents in highways is crucial to averting major traffic congestion. While recent supervised machine learning methods offer solutions to incident detection by leveraging human-labeled incident data, the false alarm rate is often too high to be used in practice. Specifically, the inconsistency in the human labeling of the incidents significantly affects the performance of supervised learning models. To that end, we focus on a data-centric approach to improve the accuracy and reduce the false alarm rate of traffic incident detection on highways. We develop a weak supervised learning workflow to generate high-quality training labels for the incident data without the ground truth labels, and we use those generated labels in the supervised learning setup for final detection. This approach comprises three stages. First, we introduce a data preprocessing and curation pipeline that processes traffic sensor data to generate high-quality training data through leveraging labeling functions, which can be domain knowledge-related or simple heuristic rules. Second, we evaluate the training data generated by weak supervision using three supervised learning models -- random forest, k-nearest neighbors, and a support vector machine ensemble -- and long short-term memory classifiers. The results show that the accuracy of all of the models improves significantly after using the training data generated by weak supervision. Third, we develop an online real-time incident detection approach that leverages the model ensemble and the uncertainty quantification while detecting incidents. Overall, we show that our proposed weak supervised learning workflow achieves a high incident detection rate (0.90) and low false alarm rate (0.08).

==> Traffic incident detection/1-intro.tex <==



Traffic congestion negatively impacts quality of life and economic productivity, causing longer travel times and loss of productivity \cite{falcocchio2015costs}. According to the U.S. Department of Transportation \cite{systematics2005traffic} 
%\PB{cite?},\YS{the name of cited website was USD, changed to the web address} 
25\% of traffic congestion stems from the direct consequence of traffic incidents. Moreover, traffic incidents can cause secondary incidents that lead to additional property loss, injury, and even death. Therefore, a fast and reliable traffic incident detection system is needed to detect incidents quickly and accurately so that traffic management controllers can make adjustments in real time to redirect traffic. Achieving accurate automated incident detection (AID) has been a research topic for decades. With the help of increasingly abundant data describing traffic conditions, data-driven methods for incident detection have been developed. These methods seek to provide fast and accurate traffic incident detection with a high detection rate (DR) and low false alarm rate (FAR). Specifically, methods based on time series analysis and machine learning (ML) have  become the most popular for their ability to explore the temporal relationships among traffic variables and the potential of utilizing hidden patterns within the traffic data.

Real-world traffic data are  noisy and  challenging to curate for pattern extraction. Traffic patterns can vary with different road conditions, weather, and time of the day, making detection of incidents difficult.  The most commonly used data for data-driven incident detection are inductive loop detector measurements. Not only are the measurement values  dependent on the detector condition, but also their use must account for localized road geometry (e.g., number of lanes, entrances, exits, intersections). Moreover, the distance between adjacent loop detectors is not uniform, a situation that, depending on the distance between the detectors, can result in pattern shifts between detectors. For incident detection tasks in particular, the success of data-driven models  greatly depends on the reported incident events, which do not always match well with the observed traffic condition.
%, shown in Figure \ref{miss-label}. %\PB{this is not clear} \YS{referred to the figure} 
%GAIL - you shouldn't refer to a figure that is pages away  and especially  when you have not referred to  figs 1-4 yeert.s
Therefore, careful treatment of the real-world traffic data is required for the data to be useful for AID.  %\PB{what do you mean by continuous work?} -- \YS{changed}.

Previous studies on AID using ML methods  focused mainly on using and improving different models to achieve better detection. However, the impact of the quality of the data  used to train the models was overlooked---even though the correctness of the training data fundamentally determines the performance of a data-driven model, regardless of the model complexity. %\TM{why the focus changed?} -- \YS{added transition}. 
In recent ML approaches, data quality has gained increasing attention  as  a major driving force for a successful machine learning model. Researchers are recognizing that high-quality training data is required in order to perform prediction with high accuracy \cite{gudivada2017data}. 

In this paper we introduce a data-centric workflow that processes raw incident data collected from the Performance Measurement System (PeMS) database \cite{chen2002freeway}, and we generate high-quality training data using a weak supervision technique. The data generated by this technique are further utilized by a number of machine learning models as the high-quality training set. Our evaluation shows that the high-quality training data improve the model accuracy significantly and greatly reduce the FAR introduced by seemingly 
incident-related traffic patterns during normal traffic conditions. Further, we  perform uncertainty quantification for AID using deep ensemble. 
As the first work on incident detection using the data-centric approach, the contributions of this study are as follows.
(1) Data-centric modeling is emphasized.  High-quality data are generated via weak supervision. The training set created by weak supervision requires no feature engineering. 
(2) The importance of data preprocessing and curation is discussed and presented by comparing the performance of models with the same architecture trained on different levels of treated data. 
(3) The importance of the quality of the training data on the model performance is shown by evaluating the training data generated via weak supervision using three machine learning models---random forest, k-nearest neighbors (KNN), and support vector machine (SVM) ensemble---and long short-term memory (LSTM) classifiers. To the best of our knowledge, this is the first application of LSTM to detector-level traffic incident detection with only loop detector measurements. 
(4) Our uncertainty quantification for AID is helpful for understanding whether the model prediction is trustworthy or not.
%GAIL - shouldn't this next sentence go with your first point? I realize you say Overall, but it still seems out  of  place after UC  and weak supervision 
%Overall, this is the first work on incident detection using the data-centric approach. -- added in the paragraph

%Data-driven models require high-quality training data to perform prediction with high accuracy \citep{gudivada2017data}. High-quality, labeled data is essential for successful incident detection. 


%In this work, we introduce a data-centric workflow that processes raw loop detector measurements, selects high-quality data, and uses an ensemble of recurrent neural network with uncertainty quantification for AID. This detection workflow aligns well with realistic scenarios and could greatly reduce the FAR introduced by seemingly incident-related traffic patterns during normal traffic conditions. The contribution of this study is 3-fold: \PB{I would change the order; emphaize the weak supervised learning first, then ensemble RNN with UQ for incident detection, say no feature engineering is required!}-\YS{changed} 1) data-centric modeling is emphasized and data curation is achieved via weak-supervision. We should by using the training set created by weak supervision, there is no feature engneering neede. The importance of data preprocessing and curation is discussed and presented by comparing the performance of models with the same architecture trained on different levels of treated data; 2) to the best of our knowledge, this is the first application of RNN to detector-level traffic incident detection with only loop detector measurements; 
% and 3) the calculations of AID performance metrics (DR, FAR) with clear interpretation are determined, providing a consistent evaluation process for future studies \
%\PB{this is not a contribution}. -\YS{took it out} 

%The rest of the paper is organized as follows. Datasets used in the study and their treatment for being ML ready are described in Section \ref{data}. The data curation process, the RNN-based time slices classifier, model hyper-parameter search, and deep ensemble are presented in Section \ref{method}. In Section \ref{results}, we show the effect of data curation on improving classification performance of three different models, the visual interpretation of the proposed RNN-based model with saliency maps, traffic incident detection results of the RNN-based model and the deep ensemble model with uncertainty measure, and the process of real-time incident detection with the proposed method. The previous studies on network-level AID and senor/link-level AID with machine learning techniques are reviewed in Section \ref{related}. Finally, the summary, limitation of this work, and our vision for the future work can be found in Section \ref{con}.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{images/incident_pattern_new.png}
    \caption{Traffic incident pattern schematic (\cite{motamed2016developing}). During a traffic incident, the corresponding upstream and downstream loop detectors will measure different traffic patterns. The expected response is a decrease in upstream speed and volume and in downstream volume, with an increase in upstream occupancy and changed downstream speed and occupancy. %\PB{where is this figure reffered in the text!} \YS{it is referred in section 2. Moved this figure to data tex file}
    }
    \label{schematic}
\end{figure}

==> Traffic incident detection/2-data.tex <==




Loop detector measurements of traffic data and incident data were downloaded from the Caltrans Performance Measurements System (PeMS) database \cite{chen2002freeway}. The data were collected from  detectors spanning the entire California freeway system across all major metropolitan areas. %\PB{if we are not using  40,000, then we should not say that; focus on only I-80 sensors and data volume} -\YS{changed}% \PB{cite} \PB{also add a description of what it is; you have to say it california highway etc}. 
From this dataset, a section  of detectors on I-80 East in Caltrans District 4  were arbitrarily selected for analysis. 
%\PB{Why this particular data set; say that this was used in the previous studies!?} -- \YS{we just randomly selected this region and road to limit the scope} 
The data in the training set spanned 3 months and were sampled from January to March 2019. The validation set came from April and May 2019. The data from the rest of the year 2019 (June--December) were used as the testing set. 
% The sensor-level incident detection is largely dependent on traffic local behavior, for only minutes' of history was to be used in model training. Therefore, in order to enrich the training set, the information of the same months of different years was gathered to create the training set 
%\PB{not clear; previously you said you used only January to March of 2019}. -\YS{this is an oversight, the sentence is deleted} 
There was no time overlapping between the training, validation, and testing sets. Training and model tuning %\PB{not clear what you mean by evaluation} \YS{changed to model tuning}
were done on the training and validation set. 
The incident detection was done on the testing set. 

%  To increase the size of the model training set and to avoid introducing effects of seasonal dynamics, the information of the same months of different years were combined to create the training set which included January, February of 2019, and January, February, and March of 2020. The validation set included March, April, and May 2019. The data from the rest of 2019 (June - December) were used as the testing set. As such, these three distinct datasets provided the foundation for model development.
 
 %The incident detection was done on the testing set. Classifier training and evaluation were done on the training and validation set. \PB{You have to argue that there is no data leakage from test to training data set; this is critical and not clear from the current text}. -- \YS{added}

%Incident detection largely depends on localized behavior. %\PB{not clear what do you mean by localized behaviour?} 
%GAIL - I agree - what is localized behavior here? In psychology it refers to  different parts oft he brain being  responsible for different actions.  Do you mean driving  behavior, like  risk? And how  does this connect with traffic  dynamics? In addition, incident-related traffic dynamics occur over a period of time. As such, our detection model focuses on learning the time series signatures of the traffic dynamics. %\PB{rewrite this sentence; not clear} -- \YS{need help}. 
The traffic dynamics are captured by inductive loop detectors. Loop detector measurements include speed, volume, and occupancy at a resolution of 30 seconds ($t$ indicates the time step). 
%GAIL - it seems odd to define  these symbols here  when you don't present the equation until the next subsection.Move it there?
%YS -- moved
Speed represents the average vehicle speed during a 30-second window for each lane, volume represents the number of vehicles on each lane that passed the detector, and occupancy accounts for the proportion of time during the detecting window that the detector was occupied by the vehicles. %\PB{whole paragraph does not read well!}.
%GAIL - covered by or occupied by?

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/viz_profile.png}
    \caption{Loop detector measurement changes during an incident, of which the duration is marked in pink background. The expectation is to observe speed and occupancy separation between upstream and downstream detectors and drop in volume from both detectors. More specifically, one expects an upstream speed drop and occupancy increase and a volume increase on both detectors during an incident. (a)(b) match the expectation. The volume profiles in (c)(d)(e) do not follow the expectation, nor do they follow an obvious pattern, while the speed and occupancy profiles still align with the expectation.}
    \label{pattern}
\end{figure}


In order to define an incident, an upstream detector and a downstream detector are established around the incident location. Upstream detector captures the outgoing traffic from the incident location and the downstream detector captures the incoming traffic towards the incident location. 
%GAIL - were they established? If so, should the next sentence say ... dynamics include... or should the sentence say "downstream speed would remain..."? There seems to be a mix of tense and mood here
The expected traffic dynamics include an obvious drop in the incident location's upstream speed while the downstream speed remains the same, Figure~\ref{schematic}.
% Although traffic volume and occupancy are also impacted by and incident, they are also more sensitive to the number of vehicles present which varies significantly during the day. Therefore, in our study, only speed profiles were used for incident detection. 
Although all traffic profiles have their expected pattern changes, in reality they are not always observed, especially for volume change, shown in Figure \ref{pattern}. Thus, in this work we  focus only on utilizing speed and occupancy information to detect incidents. %\PB{Both figures are not explained well} -\YS{these two paras are Jane's editing. Not sure if should change}




%\subsection{Data Preprocessing}
% The raw data were further processed and cleaned to meet the requirements to train data-driven models. A list of procedures was followed to deal with all data obtained. They are \PB{do you need this list?}:
% \begin{enumerate}
%     \item Unify timestamps of the data from each detector by linear interpolation.
%     \item Aggregate the lane speed measurements.
%     \item Forward fill the missing values of the same detector based on the timestamps.
%     \item Fill the missing values of different detectors using spline interpolation.
%     \item Filter the data along the time axis using exponential moving average.
%     \item Normalize the data by their values at free flow.
%     \item Check data quality by comparing oscillation statistics.
% \end{enumerate}
% sorry didn't put track changes on for me until I got here....
\subsection{Data preprocessing}
In order to curate the data for training a data-driven model, the raw data (speed $s^{(t)}$, volume $v^{(t)}$, and occupancy $o^{(t)}$) were further processed and cleaned. The initial step focused on aligning the timestamps of the localized detectors because the detectors operate asynchronously %\TM{what does it mean?}. -- \YS{I think this is Jane's take on the fact all measurements do not have the same timestamps}. 
%In order to align the data in time, 
Specifically, linear interpolation was used to assign the corresponding values to the desired timestamps. In addition, speed values were reported for each lane ($s_1, s_2, \dots, s_n$); however, the number of lanes $n$ was not constant. Therefore, in  order to reduce the complexity of the problem, the lane information was aggregated as the volume-weighted average of all lanes. %\TM{formula} 
\begin{linenomath*}
$$ s^{(t)} = \frac{\sum_i^n s_i^{(t)} v_i^{(t)}}{\sum_i^n v_i^{(t)}}$$
\end{linenomath*} 
Furthermore, to deal with missing values, we adopted two different methods. First, for the same loop detector, the missing values were filled with the nearest available value at the previous timestamp. Second, for detectors that had missing values at the first timestamp (e.g., 01-02-2019 00:00), the values were filled with a spline interpolation of spatial locations of consecutive detectors, under the assumption that two adjacent detectors share a similar traffic pattern. 

As with any real-world device, it was not uncommon to see  values that were clearly unrealistic, for example, speed values that were too high for the physical situation. In order to address such situations, an exponential moving average with a step size of 5 (2.5 minutes) was utilized to smooth the 30-second resolution time series data: 
\begin{linenomath*}
$$s^{(t)} \leftarrow \frac{\sum_{j=0}^t w_{j} s^{(t-j)}}{\sum_{j=0}^t w_j}$$
\end{linenomath*}, where $w_j = (1 - \alpha)^j$ is the weight associated to the value at step $j$ ahead of the current time $t$, $\alpha = 0.33$ is the decay factor calculated based on the moving window size 5 (2.5 minutes), and $s^{(t)}$ is the aggregated speed values at time $t$, 
%GAIL - are the aggregated speed values only  the s^{(t)}$'s or the alphas also? That is, I am uncertain whether the following sentence abpit they are updated refers just to the s^{(t)}$'s. If it does, perhaps  say $\alpha = 0.33$, and $s^{(t)}$'s are...at time t and are updated...
and they are updated by the rule above. The same moving average process was applied to occupancy $o^{(t)}$ and volume $v^{(t)}$.
This approach was helpful for revealing the underlying pattern of the time series data and increasing the robustness of detection models. 

Knowing the sensitivity of data-driven models to the quality of the data, we applied an additional filtering step. Because normal data sequences with 30-second resolution usually still exhibit oscillations after smoothing, we assumed that low-quality data would appear as flat lines or extremely smooth curves, and we filtered these data points from the model training and evaluation dataset. This quality check filter was implemented by comparing the mean of the numerical first derivative of each traffic profile to the same statistics from the training set. This method is based on the assumption that the oscillation of normal traffic profiles follows a similar pattern with limited deviation. %\TM{intuition} \YS{added}. 
Take speed $s^{(t)}$ as an example. Within a certain time span (e.g., 3 hours), we calculate the numerical first derivative $s'^{(t)}$ and take the mean over the time span as $\bar{s'} = \frac{1}{T}\sum_{t=0}^{T}s'^{(t)}$. This process is repeated for all the examples in the training set. We then take the sample mean and standard deviation of all $\bar{s'},$ 
\begin{linenomath*}
$$\mu_{\bar{s'}} = \frac{\sum_k^m \bar{s'}_{k}}{m},$$ 
$$\sigma_{\bar{s'}} = \frac{\sum_k^m s'_k - \mu_{\bar{s'}}}{m},$$
\end{linenomath*} 
where $m$ is the number of data points in the training set. 
%\jm it this correct for the three profiles? 
For new traffic profile series, the mean of the numerical first derivative $\bar{s'_{new}}$ will be compared with $\mu_{\bar{s'}} \pm \sigma_{\bar{s'}}$. If $\bar{s'_{new}}$ lands in the range, the new data point is considered to have good qualify; otherwise, it will be considered to have bad quality and will be taken out. 
% is  we calculate the first derivative sequence of each profile, then take the mean of the first derivatives. If the mean values are within one standard deviation of the training set, the new profiles are considered good quality, and are used for incident detection. 
An example of low-quality data is shown  in Figure \ref{low_quality}, where both data points exhibit data with little variation. The left figure shows a situation in which both upstream and downstream sensors are reporting low-quality data. The right figure indicates that a downstream detector is reporting low-quality data.

%\PB{a question will be how these preprocessing will be applied during the model deployment?}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/lowqual.png}
    \caption{Examples of low-quality data. }
    \label{low_quality}
\end{figure}

\subsection{Labeled incidents}
PeMS includes reports of incidents from traffic management centers or the California Highway Patrol that will provide labels for the associated traffic profiles. Incidents are characterized by incident location, incident starting time and duration, and incident type. Figure \ref{low_quality} includes the reported incident data by showing a shaded bar that indicates the start time and duration of the incidents. Reported incidents in the database are created for a variety of traffic situations, and not all of the reported incidents are captured by loop detector measurements.  For this study, only the incident data that were categorized as accidents and showed evidence of change at the detector level were extracted and matched with loop detector measurements. % accordingly to the information described above. \PB{where did you get the incident information? you have to say that} -- \YS{mentioned}

==> Traffic incident detection/3-method.tex <==
% During a traffic affecting incident, the traffic speed profiles are expected to have a drop on the upstream and maintain the downstream values while the occupancy of upstream increases. For each timestamp, it has two possible outcomes--belongs to an incident or not.
% %within \PB{what do you mean by during?} -- \YS{changed to within an incident duration} an incident duration or not. 
% It is natural to classify each timestamp based on the corresponding speed profiles to detect incidents. However, the preprocessed loop detector measurement data was not ready for effective model training due to the considerable miss-labeling issue. Also, the duration of incidents could vary and multiple timestamps could belong to a single incident. Thus, it is unreasonable to count individual times slice into the total numbers of incidents and non-incidents. In this section, we first describe the data curation criterion and process of creating high quality data for model training,  then we describe the default classification model for classifying time slices as well as the incident detection criteria after classification, and finally we introduce a real-time detection approach for detecting sensor-detectable cases with our methods.


Our approach comprises three key steps:  determine the data curation criterion and process of creating high-quality data for model training, develop a classification model for classifying time slices and the incident detection criteria after classification, and design a real-time detection approach that will fully identify and classify sensor-detectable cases.%\PB{we should first talk about the workflow; here you are direclty entering into the detection. The whole point is the data curation, which you did not even mention here}. --\YS{added. I overlooked the old section overview. Also moved the lstm classification process figure to the classification section}

In the supervised learning setting, with the input-output pair $\mathbf{x}$ and $Y$, the model input was prepossessed with traffic speed and occupancy time series data 
\begin{linenomath*}
$$\mathbf{x} = (\{s^{(t-h)}, \dots, s^{(t)}\}, \{o^{(t-h)}, \dots, o^{(t)}\})$$
\end{linenomath*}
, where $h$ is the measurement history taken into consideration. The model output was to approximate the gold label 
\begin{linenomath*}
$$Y \in \{0, 1\}$$
\end{linenomath*}, where 0 represents a non-incident label and 1 represents an incident.

%within \PB{what do you mean by during?} -- \YS{changed to within an incident duration} an incident duration or not. 
 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/workflow.pdf}
    \caption{RNN-based incident detection workflow. (a)  Data preprocessing and curation processes, in which the raw station data are first made machine learning ready and then labeled via weak supervision. (b) Data flow in the neural network. The time series data were fed into RNN layers and then into fully connected layers for classification. (c) Process of the model classifying time slices and detection being made.} %\PB{why LSTM?} -- \YS{mentioned in the corresponding section}}
    \label{workflow}
\end{figure}

\subsection{Data curation}
The two datasets described in the preceding section provide the foundation for the approach: the inductive loop measurements that provide the speed profiles at specified locations on the road network, and the associated labeled incident data. Field data were cleaned and smoothed to provide quality data; however, the labeled incident data had significant issues. Challenges included incorrect incident start and end times, as well as incident location overlaps in which a detector is capturing the dynamics of multiple events.
% is this correct?
%We have expectations on the change of speed profiles when an incident happens. Nonetheless, %However, the pre-processed loop detector measurement data was not ready for effective model %training due to the considerable mislabeling issue. Also, the duration of incidents could %vary and multiple timestamps could belong to a single incident. Thus, it is unreasonable to %count individual times slice into the total numbers of incidents and non-incidents.

A traffic-affecting incident profile is expected to have a drop on the upstream speed, while maintaining the downstream speed, and an increase in the upstream occupancy. For each timestamp, two outcomes are possible---it belongs to an incident or not. However, the impact of an incident on speed profiles can be diverse. Many times when an incident happens, it has minimal influence on the traffic, for example, an incident that occurs at night  when  fewer vehicles are on the road.  %\PB{when that happens?} -- \YS{metioned night time when number of cars is few}.
In this work we focus only on detecting incidents that are sensor detectable, meaning that there was an observed difference between upstream and downstream speeds. The majority of these cases presented a significant drop in the upstream speed and unchanged downstream speed. Road conditions can be complicated, however, and unexpected scenarios can happen. For example, several cases showed upstream and downstream separation where the downstream speed was much lower. Also, in some cases  both upstream and downstream speed profiles had an abrupt drop during an incident. These cases showed a steeper drop and tended to last for a shorter period of time than peak-hour-related traffic profiles. All the sensor-detectable cases described  were selected from the original training set for model training. 

As mentioned, the labeling associated with the sensor-detecable cases was not accurate. A recurring inaccuracy was that the reported incident starting time and duration did not match the traffic profiles. Figure \ref{miss-label} shows an example of poorly labeled sensor data. Using the incident reports directly with the original labels would greatly confuse the models and lead to poor classification performance.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/miss-labeing.png}
    \caption{Mislabeled time slices with traffic profiles. The red background indicates the reported accident duration. The speed profiles of the circled areas do not match the reported incidents.}
    \label{miss-label}
\end{figure}

% To take out the miss-labeled instances, dataset cartography was used to categorize the training data points. The idea is to get the training dynamics for each training data point from each epoch. Three statistics are calculated from the training dynamics of each data point, namely, confidence, variability, and correctness. Confidence is defined as the mean of true label probability, variability is the standard deviation of the model output true label probability, and correctness is the number of time the model makes the right prediction, shown in Equations \ref{conf} \ref{var} \ref{cor},

% \begin{align}
%     confidence &= \frac{1}{n}\sum_{i=1}^{n}p_{t}^i \label{conf}\\
%     variability &=\sqrt{\frac{1}{n}\sum_{i=1}^{n}(p_t^i - \Bar{p_t})^2} \label{var}\\
%     correctness &= \frac{\# \text{ times of correct classification}}{\text{\# epochs}}
%     \label{cor}
% \end{align}
% where $n$ is the number of epochs set for training process, $i$ indicates the $i$th epoch, and $p_t$ is the true label probability from the model. Based on these statistics, training data points can be put into easy-to-learn, ambiguous, and hard-to-learn categories. Easy-to-learn data are those with high confidence and low variability, from which the model can relatively easy to learn and thus make the correct predictions. Ambiguous and hard-to-learn instances often have low confidence, for which the model is not able to make right prediction the majority of the times. In this work, we selected training points with correctness greater than 0.5 (the model can make the right prediction more than half the time) and took out the rest instances (mostly associated with ambiguous and hard-to-learn data).

% \paragraph{Manual data selection}
% A manual approach for generating labeled data was deemed necessary in order to manage the mislabeling of the incident data. This required defining detectable features in the data that could consistently identify both classifications: incident and non-incident. As shown earlier, the candidate measurements for this were the upstream speed and the downstream speed.
% \begin{itemize}
%     \item Non-incident: Near zero separations between the upstream and downstream profiles indicated the continuity expected in normal traffic dynamics.
%     \item Incident: Clear separation between the upstream and downstream speeds.
% \end{itemize}

% The manually selected training set contained 1181 data points (593 non-incident and 588 incident slices) and the validation set 457 data points (235 non-incident and 222 incident slices). Figure \ref{handpick} shows the manually picked instances for model training and validation.

%However, due to changes in the road layout, a good portion of data that presented a clear separation between the upstream and downstream speed were not labeled as an incident. This conflicting information in the training set would result in models with poor performance, regardless of the expressive power of the models.  To address the mislabeling issue in the training set, time slices were manually selected based on  10-minute histories and correct labels were applied. 

%-----------------------------
% add snorkel part
%-----------------------------
\paragraph{Creating training set with weak supervision}
%\PB{we need to provide more details on the weak supervision; mathematical details of how the weak labels are combined but applied to our problem. Currently, this is missing! Note that this is one of main contribution of the paper} \YS{added: the details are quite complicated and I do not fully understand yet. But I listed out the overall process}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/snorkelFlow.pdf}
    \caption{Probabilistic labels creation process using Snorkel. The unlabeled data points get labeled by a set of labeling functions $L_1, \dots, L_n$. The $i$th labeling function produces a label $\lambda_{i, j}$ or abstain for data point $j$. Snorkel then evaluates the labeling function accuracies without accessing the true label and produces probabilistic labels, which can be used directly in the downstream classifier.}
    \label{snorkel}
\end{figure*}




 Weak supervision uses the information from different weak labelers to create high quantity and quality of training data. These labelers can be noisy and imprecise, however, and usually follow a set of rules that are manually determined. In this work we adopt \texttt{Snorkel} \cite{ratner2017snorkel}, a system for quickly generating training data with weak supervision, to label our training set based on a set of labeling functions (LFs). The LFs determine whether a particular data point should be labeled as incident, non-incident, or abstain based on individual criteria. \texttt{Snorkel} produces labeling statistics from all LFs and then leverages the importance of each LF by inspecting the coverage and conflicts of all LFs. It then outputs probabilistic labels for the labeled data points in the training set, encoding the noise brought by the LFs. In essence, \texttt{Snorkel} models the joint probability distribution \begin{linenomath*}
$$p(\lambda, Y),$$
 \end{linenomath*} where $\lambda$ is a vector containing the results from all LFs and $Y$ is the gold label (ground truth), and outputs the conditional probability $p(Y | \lambda)$ as the probabilistic labels for the data points, as shown in Figure \ref{snorkel}. \texttt{Snorkel} is able to quickly model the joint distribution and estimate the accuracy of the LFs without knowing the gold label $Y$, which is done via solving a matrix-completion-style problem \cite{ratner2019training}. More specifically,  a user can define a source graph $G_{source}$ capturing the dependencies between LFs. If no such graph is provided, \texttt{Snorkel} will treat LFs independently conditioned under the true labels and learn the correlation during the process. To model $p(Y|\lambda)$, \texttt{Snorkel} parameterizes the distribution with a vector of source (LFs) correlations and accuracies $\mu = \mathbb{E}[\psi(C)]$,
 where $\psi(C) = \{0, 1\}^{\prod_{i\in \mathcal{C}}(|\mathcal{Y}_i| - 1)}$, $C \in \mathcal{C}$, $\mathcal{C}$ is the set of cliques of $G_{source}$, and $\mathcal{Y}_i$ is the output space from the $i$th source. \texttt{Snorkel} estimates $\mu$ without  access to the true labels, by analyzing the covariance matrix of the cliques in $G_{source}$. The set of the cliques in $G_{souces}$ can be written as $R \cup Q$, where $R$ is the observable cliques and $Q$ is the separator set of cliques. 
 %GAIL - do you separator set of cliques
 of the junction tree of $G_{source}$. Thus, the random indicator variables $\psi(C) = \psi( R \cup Q)$, and 
 \begin{linenomath*}
$$\mathbf{Cov}[\psi(R \cup Q)] = \begin{bmatrix}
	\Sigma_{R} & \Sigma_{RQ}\\
	\Sigma^T_{RQ} & \Sigma{Q},
\end{bmatrix}$$
which has the inverse
$$K = \mathbf{Cov}[\psi(R \cup Q)]^{-1}=\begin{bmatrix}
	K_{R} & K_{RQ}\\
	K^T_{RQ} & K_{Q}
\end{bmatrix}.
$$
 \end{linenomath*}
 
Here, $\Sigma_R$ is known, and $\Sigma_S$ is known or can be estimated. The source correlations and accuracies $\mu$ can be recovered by obtaining $\Sigma_{RS}$. One can show that if  $z = \sqrt{c}\Sigma_{R}^{-1}\Sigma_{RQ}$, where $c = (\Sigma_Q -\Sigma^T_{RQ}\Sigma_R^{-1}\Sigma_{RQ})^{-1}$, then
\begin{linenomath*}
$$K_R = \Sigma_R^{-1} + zz^T$$
\end{linenomath*}
in which $K_O$ is determined by $G_{source}$ , $\Sigma_R^{-1}$ is observable, and $zz^T$ can directly solve for $\mu$ via an algorithmic approach that treats estimating $z$ as a matrix completion problem. More details of the development and analysis of this method are in the original work \cite{ratner2019training}.

For traffic incident detection, given the observations shown in Figure \ref{pattern}, we designed 10 LFs %\PB{you have to be precise here} \YS{added the number} 
related to speed and occupancy as the weak labels to create the training set with probabilistic labels. The LFs are based on speed and occupancy changes (separations, single- or double-sided drop or increase) during an incident. Examples of LF function results with incident labels are shown in Figure \ref{LFs}. In total, 157,430 time slices were labeled by \texttt{Snorkel}, among which 118,054 were non-incident slices and 39,376 were incident slices. %\YS{add how many data examples from snorkel dataset}

\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{images/snorkel_LF.pdf}
\caption{Incident examples based on labeling function results for Snorkel. (a)--(d) show the speed-based labeling function results. Specifically, (a) shows upstream and downstream separation; (b) shows more significant separation; (c) presents one-sided speed drop; and (d) shows double-sided speed drop. Similarly, (e)--(f) show the labeling function results based on occupancy. 
%(e) and (f) show the occupancy separation, 
(g) shows single-sided occupancy increase, and (h) shows the double-sided occupancy increase. }
\label{LFs}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/handpick.png}
%     \caption{Examples of manually selected instances based on 10-minute history. (a) shows the non-incident data points where the upstream and downstream speed profiles follow the same trend and the relative speed difference is near near 0. (b) shows the incident data points. The first row shows the most common scenario in which the upstream speed is lower than the downstream speed; the second row shows the reversed profile where the downstream speed decreases during an incident; the third row shows the abrupt change of the upstream speed.}
%     \label{handpick}
% \end{figure}

% \paragraph{Feature extraction}
% Since most of the human detectable cases were based on the separation between the upstream and downstream speed, the relative speed difference between the loop detectors was extracted as shown in Equation \ref{rel_speed}. 
% \begin{align}
%     \delta_{rel} = \frac{u_{down} - u_{up}}{0.5(u_{down} + u_{up})}
% \label{rel_speed}
% \end{align}
% The extracted relative speed difference has both a lower bound and an upper bound, and thus it is beneficial for model training for the relative speed is comparable throughout the instances. 

\paragraph{Offset upstream speed}
Manually selected non-incident data points had non-separable or close to non-separable upstream and downstream speed profiles. In reality, because of complex road conditions and non-uniform distances between upstream and downstream loop detectors, a constant separation may occur between the speed profiles, shown in Figure \ref{offset}. The models will perform poorly on the non-incident time slices in these cases. To address this issue, we offset the upstream speeds  by the one-hour average speed difference of the downstream speeds, effectively normalizing the speeds.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/offset.png}
    \caption{Offset of the upstream speed with one-hour average speed difference during normal traffic. (a) Original speed profiles; (b) profiles with upstream offset.}
    \label{offset}
\end{figure}


\subsection{Time slice classification}
A recurrent neural network (RNN) classifier with long short-term  memory  %\PB{is this defined?}
cells was adopted because of their success and popularity in sequential learning tasks. %LSTM networks \citep{article} are a type of recurrent neural network that controls the long or short-term memory of the network by using gates of characteristic data.
The LSTM network acts as the default model for classifying individual time slices into incident and non-incident classes.  For the AID task, it is important to capture not only the instantaneous behavior of the traffic profiles but also the changing trend of the profiles with time. In this implementation, the LSTM layers take into account the information from the history (10-minute history in the default setting) for each speed profile and return the final state for classification. Classification was achieved by the final dense layers. With the sigmoid activation at the final layer, the  network  outputs the probability values of each time slice being an incident time slice. 

% \PB{fix this part!} -- \YS{not sure what}
%GAIL - I am not sure what you mean by the last two sentences - sigmoid activation and how classification is achieved by the following dense layers

%The basic building blocks of such a network are called LSTM cells, with each consisting of an input node, an input gate, a forget gate, an output gate, a state unit, and a self-loop unit. The data flow in an LSTM cell is defined as follows \cite{Goodfellow-et-al-2016}:

% \begin{align*}
%     i_i^{(t)} &= \sigma(b_i^g +\sum_j U_{i,j}^ix_j^{(t)} + \sum_p W_{i,p}^gh_p^{(t-1)})\\
%     f_i^{(t)} &= \sigma(b_i^f +\sum_j U_{i,j}^fx_j^{(t)} + \sum_p W_{i,p}^fh_p^{(t-1)})\\
%     s_i^{(t)} &= f_i^{(t)}s_i^{(t-1)} + g_i^{(t)}\sigma(b_i +\sum_j U_{i,j}x_j^{(t)} + \sum_p W_{i, p}h_p^{(t-1)})\\
%     g_i^{(t)} &= \text{tanh}(b_i^g +\sum_j U_{i,j}^gx_j^{(t)} + \sum_p W_{i,p}^gh_p^{(t-1)})\\
%     h_i^{(t)} &= \text{tanh}(s_i^{(t)})q_i^{(t)}\\
%     q_i^{(t)} &= \sigma(b_i^o +\sum_j U_{i,j}^ox_j^{(t)} + \sum_p W_{i,p}^oh_p^{(t-1)})
% \end{align*}
% where $\mathbf{x}^{(t)}$ is the input vector of current time, $\mathbf{h}^{(t)}$ is the output or short-term state vector of current time, $\mathbf{s}^{(t)}$ is the long-term state vector of current time and $\mathbf{U}$, $\textbf{W}$, $\mathbf{b}$ are weight matrices for the input vector, weight matrices for short-term states, and bias terms, respectively. 

%The LSTM cells are connected recurrently, taking the input vectors one step at a time. An LSTM layer consists of one or more such LSTM cells and returns the final state vector of the input. In the LSTM classifier, the final state vector is further fed into a few dense layers which finally output the class probability via a logistic activation function (sigmoid function). 

% The loss function of choice for model training was  binary cross-entropy (BCE). BCE is widely used in binary classification problems with probability output. To avoid a class imbalance problem for supervised learning, the a balanced selection of manually selected training and validation sets were definied. We found BCE could suffice to serve as both the loss function and hyper-parameter search objective in this work. The workflow of the RNN-based \PB{LSTM or RNN?} -- \YS{fixed} incident detection is shown in Figure \ref{workflow}. 

The loss function of choice for model training was focal loss (FL) \cite{lin2017focal} due to the class imbalance nature of the problem. It is defined as follows: 
\begin{linenomath*}
$$FL = -(1 - p_t)^{\gamma}log(p_t)$$
\end{linenomath*}, where $p_t$ is the true label probability. FL puts more importance on the harder-to-learn examples that usually are the data points with minor class labels. The parameter $\gamma$ was set to be the default value from its original work \cite{lin2017focal}. We found FL could suffice to serve as both the loss function and the hyper-parameter search (HPS) objective in this work. The workflow of the data-centric RNN-based incident detection is shown in Figure \ref{workflow}. 

% \begin{align}
%     BCE = -p_tlog(1 - p_t)
% \label{bce}
% \end{align}

% Due to the imbalanced nature of traffic incident datasets, a loss function named focal loss \cite{lin2017focal}, was adopted to level the importance of the minority class instances during neural network training. The focal loss was originally designed for object detection in computer vision tasks, where the object area would be much smaller than the entire image. Similarly, the focal loss can be used in training classifiers when the training label distribution is imbalanced with the number of positive instances much less. Focal loss is defined as follows. 

% \begin{align}
%     FL = -\alpha y(1-p)^{\gamma}log(p) - (1 - \alpha)(1 - y)p^{\gamma}log(1-p)
% \end{align}

% where $y$ is the true label and $y \in \{0, 1\}$, $p$ is the prediction probability for the positive class, $\alpha$ is the weighing factor, and $\gamma$ is the power to the modulating factor. The modulating factor makes the easily classified instance contribute less to the overall loss, which in turn increases the importance of correcting miss-classified instances. In addition, the weighing factor $\alpha$ assigns more importance when the label of the miss-classified. In this way, the model will have a larger loss when there is a miss-classification from the minority class, encouraging the network to learn the underlying mapping better. 

% \subsection{Single Event Grouping (\textcolor{red}{this will be taken out})}
% During an incident, all the time slices within should be labeled as incident slices and successive. Therefore, it is essential to group time slices to form individual incident events after classifying. There are a few rules followed in this work to label and group the LSTM network classified time slices, shown in Alg \ref{grouping}.

% \begin{algorithm}[h!]
% \SetAlgoLined
% Time slice sequence with probabilities $S_p$\;
% Set threshold $\epsilon$ for labeling\;

% \eIf{$S_p > \epsilon$\;}{
%  label slices as incidents\;
%  }{label slices as non-incidents\;}

% Labeled time slice sequence $S_l$\;
% Set grouping window size $m$\;
% Distance between two adjacent incident time slices $d$\;
% \eIf{$d>m$\;}{
% label time slices in between incidents\;
% }{pass\;}
% Incident blocks in time slice sequence $S_b$\;
% Average incident duration $\tau$\;search algorithms such as grid search, random search and
% \eIf{incident block duration $>$ average incident duration\;}{
% label the excessive part as non-incidents\;
% }{pass\;}
%  \caption{Time slices labeling and grouping}
%  \label{grouping}
% \end{algorithm}

% There are a few parameters that can vary in the grouping process. Threshold $\epsilon$ controls the cutoff value for ground truth probability. A smaller $\epsilon$ will result in more positive time slices given the same predicted probabilities. The grouping window size $m$ implies the assumption that no more than one incident can happen at the same location within $m$ minutes. The average incident duration $\tau$ is the average lasting time of incidents presented in the training set. The single event grouping process was applied to all the models used in this work to compare with them without it.



% \subsection{Metrics}
% \PB{why this section is here; this should be moved to the experimental evaluation}
% The performance of a traffic incident detection model can be evaluated via two common metrics, namely detection rate (DR) and false alarm rate (FAR). Detection rate represents the ratio of the number of correctly detected incidents to the number of ground truth incidents. It reflects the detection model's ability to capture potential characteristics of an incident. On the other hand, the false alarm rate is interpreted as the proportion of falsely detected incidents among all the detected incidents. The definition of detection rate is the ratio of the number of correctly detected incidents to the number of total incidents, shown in Equation \ref{dr}. However, definitions of detection rate were not consistent in the literature. In \citep{el2018fuzzy} the numerator in the equation appeared to be the number of detected incidents. This is problematic because the number of detected incidents could potentially exceed the total number of incidents when the model makes many false detections. 

% Another important metric is the false alarm rate (FAR), which is defined in Equation \ref{far}. The inconsistency in the literature definitions also applied to FAR where the number of non-incident cases was in the denominator  \citep{xiao2019svm, zhu2018deep}. This would lead to a low FAR since the number of non-incident cases is usually much larger than that of incidents.

% We believe the following metrics are most reasonable for AID studies. The metric scores in in the results section were calculated according to Equation \ref{dr} and \ref{far} \PB{You introduce 1 and 2 here but refer to them in the previous paragraph}.

% \begin{equation}
%     DR = \frac{\text{Number of correctly detected incidents}}{\text{Number of total incidents}}
%     \label{dr}
% \end{equation}

% \begin{equation}
%     FAR = \frac{\text{Number of falsely detected incidents}}{\text{Number of detected incidents}}
%     \label{far}
% \end{equation}




Ideally, a DR of 1.0 and an FAR of 0.0 indicate a perfect incident detection model. Usually, however, there is  a trade-off between DR and FAR, where a high DR is accompanied by a high FAR. The reason is that a model tends to overdetect in order to keep up with the high detection rate, and vice versa. Thus, the objective of an incident detection model is to extract the hidden traffic incident patterns and increase DR, reducing FAR to the largest extent. 


The detection model in our work is time slices, classification based with additional detection criteria described in Section \ref{results}. % \PB{need to expand this} -- \YS{mentioned classification based with additional criteria} 
The final DR and FAR are directly related to the classifier performance. The metric used to evaluate the performance of classifiers is the F1 score, which is the harmonic mean of precision and recall. 
%Precision is the ratio of true positives to the sum of true positives and false positives, which describes how much among the classified positive instances are actually positive. The recall is the ratio of true positives to the sum of true positives and false negatives, which shows how much among all the ground truth positives can be captured by the classifier.
Similar to DR and FAR, there is usually a trade-off between precision and recall, where a higher-valued one is accompanied by a lower-valued one. In this work, high values for both precision and recall are desired. Hence, the F1 score $(\frac{2(\text{Precision} \times \text{Recall})}{\text{Precision} + \text{Recall}})$ was utilized to evaluate classifiers, being able to combine both and weigh their contributions.

\begin{comment}
\begin{align}
    \text{Precision} &= \frac{\text{True Positives}}{\text{True Positives} + \text{False Positives}}\\
    \text{Recall} &= \frac{\text{True Positives}}{\text{True Positives} + \text{False Negatives}}\\
    \text{F1} & = \frac{2(\text{Precision} \times \text{Recall})}{\text{Precision} + \text{Recall}}
    \label{clf-metric}
\end{align}
Equation \ref{clf-metric} shows the definition of the F1 score. A higher F1 score implies  better overall performance of a classifier. 
\end{comment}

\subsection{Uncertainty quantification using deep ensemble}
%Developing an uncertainty measure is critical for applying developed machine learning models to real-world scenarios. Understanding the uncertainty requires an evaluation of the model confidence when making predictions on new data points, particularly for those that are out-of-distribution (OOD). We expect the trained model to show lower confidence (high uncertainty) on  predictions made for OOD data and higher confidence (low uncertainty) on data similar to training examples (in-distribution samples). To quantify the model predictive uncertainty, a deep ensemble approach \citep{lakshminarayanan2016simple} was used. By training the model with 50 different random seeds, selecting well-performing models (classification accuracy $>$ 0.9), and then using the mean and standard deviation of predictions from those models and statistical measure of uncertainty can be obtained.  \PB{poor exposition! You need to explain the deep ensemble approach with proper notations etc @Tanwi: You can write this section with appropriate equations} 


Measuring the predictive uncertainty is critical for using the incident detection model in practice. Uncertainty estimation helps one understand when to trust the model prediction. Bayesian neural networks are used widely to measure the predictive uncertainty. These methods are computationally expensive, however,  and require significant modification of the training procedure of the existing network. Therefore, we used an alternative approach called deep ensemble \cite{lakshminarayanan2016simple} to estimate the predictive uncertainty of our incident detection model. Deep ensemble is capable of estimating high-quality predictive uncertainty. This method is easy to implement and does not require much hyperparameter tuning. 

We used a randomization-based ensemble strategy to train an $M$ LSTM network with various initializations. The parameters of the LSTM model were randomly initialized, and the model was trained on the whole training dataset. We analyzed networks with accuracy greater than a particular threshold and treated their results as a combination of Gaussian distributions to estimate the final prediction from the ensemble predictions. We then calculated the mean and variance of Gaussian distributions using the following formula:
%GAIL - do you want to keep this paragraph in present tense (We analyze, we then calculate...If so, do you want to change the first sentence to We use a randomization -- YS: using past tense here feels more right to me.. but non-native speaker here, open to any changes. 

%\begin{equation*}

    $$\mu_*(x) = \frac{1}{M} \sum_{i=1}^M \mu_i (\mathbf{x})$$
%\end{equation*}


    $$\sigma_*^2(x) = \frac{1}{M} \sum_{i=1}^M (\mu_i (\mathbf{x}) - \mu_* (\mathbf{x}))^2 .$$


By training the model with 50 different random seeds, selecting well-performing models (classification accuracy $>$ 0.9), and then using the mean and standard deviation of predictions from those models, a statistical measure of uncertainty can be obtained.

%\TM{not finished yet}   

==> Traffic incident detection/4-results.tex <==
The following summaries the process we followed.
\begin{itemize}
    \item Downloaded PeMS data  for the entire year of 2019 and for January, February, and March 2020. A smaller region on I80 was selected for analysis.
    \item Created the training set using \texttt{Snorkel} with flow profiles (upstream and downstream speed and occupancy) from January and March 2019.
    \item Created the validation set of manually selected profiles from April and May  2019.
    \item Selected sensor-detectable sequences from June to December 2019 as the testing set.
    \item Visually identified true cases of an incident to account for mislabeling in PeMS reported incident data.
\end{itemize}

This process generated the initializing data frames for our \texttt{TensorFlow} implementation. 

The next step was to conduct  a hyperparameter search  for the recurrent neural-network-based models for incident detection. We placed a set of network architecture-related and training process-related hyperparameters into the search space. The network architecture-related parameters were RNN cell type, number of RNN layers, number of units in each RNN layer, whether it is a bidirectional RNN cell, number of dense layers, and number of neurons in each dense layer. The training process parameters were batch size, number of epochs, learning rate, sequence length, and patience for early stopping. The objective function for getting the optimal configuration was set to binary cross-entropy. 
These hyperparameters of the RNN %\PB{RNN or LSTM?} -\YS{RNN} 
network were tuned by using \texttt{DeepHyper} \cite{balaprakash2018deephyper}, a scalable neural network hyperparameter tuning package. 
%A deep learning model's expressive power and generalization ability depend on both trainable weights and model architectures. The optimal or close to optimal trainable weights can be obtained from the training process via minimizing a loss function. But the parameters that determine the model architecture, which is called hyperparameters, are usually preset by hand. This would involve numerous trials and errors as well as experiences on similar problems. In this work, we adopted hyperparameter search (HPS) that can automatically and systematically search for the high-performing combination of model hyperparameters. HPS utilizes search algorithms such as grid search, random search, and Bayesian optimization, etc, to run different guided trials in parallel and return evaluation results of the models from different trails. Finally, the high-performing model configurations can be obtained. 
The evaluation of the classification performance was done on the validation set and detection performance on the testing set.

\subsection{Impact of data curation}
In order  to evaluate the efficacy of the data curation proposed in the preceding section, in addition to the proposed LSTM network, random forest, k-nearest neighbors, and support vector machine  ensemble models were trained and evaluated on the data before and after curation. %\PB{you have to say why these methods were adopted for the experimental comparison}. -- \YS{added. the following sentence} \PB{you have to say these methods are already employed for incident detection and cite those work}. 
These classifiers could use the  same training data while having fundamentally different learning mechanisms. The models were chosen because the KNN/SVM ensemble and random forest models had been used in past studies \cite{xiao2019svm, lin2020automated} for traffic incident detection.  While the RNN-based model could capture the time dependency within the traffic profiles, the other two models would treat the profiles with 10-minute history independently as individual input features. 

The performance of the trained classifiers in terms of classifying time slices in the selected validation set is shown in Table \ref{cls_perf}. 
%All models were trained with their default configurations and the validation set at this stage was not used for model tuning. 
The results indicate a dramatic performance improvement for all models after the data curation, especially in terms of  recall on the positive (incident) instances and classification accuracy. Among the models in the experiment, the proposed RNN network and random forest model had similar performance with high accuracy, but the RNN network was able to produce better recall on non-incident samples and precision on incident samples, features that are preferred in real-world applications since they would result in a lower false alarm rate. 

\begin{table}[]
    \footnotesize
    \centering
    \caption{Time slice classification model performance on the validation set before and after data curation}
    \begin{tabular}{l|ccccccc}
        \hline
        \hline
         & \multicolumn{3}{c}{Non-incident class} & \multicolumn{3}{c}{Incident class} &  \\
         &  Precision & Recall & F1 & Precision & Recall & F1 & Accuracy \\
         &\\
         \textbf{Before Weak supervision} & \\
         \hline
         Random Forest & 0.61 & 0.94 & 0.74 & 0.87 & 0.40 & 0.55& 0.67\\
         KNN SVM ensemble & 0.58 & 0.82 & 0.68 & 0.68 & 0.40 & 0.50 & 0.61\\
         LSTM & 0.70 & 0.92 & 0.79 & 0.87 & 0.58 & 0.69 & 0.75\\
         \hline
         \vspace{2em}\\
         
         \textbf{After Weak supervision}& \\
         \hline
         Random Forest & 0.83 & 0.75 & 0.79 & 0.77 & 0.85 & 0.81 & 0.80\\
         KNN SVM ensemble & 0.81 & 0.78 & 0.79 & 0.78 & 0.82 & 0.80 & 0.80\\
         LSTM & 0.92 & 0.83 & 0.87 & 0.83 & 0.92 & 0.88 & 0.87\\
         
    \end{tabular}
    
    \label{cls_perf}
\end{table}

\begin{comment}
\subsection{Saliency maps}
The proposed LSTM network trained on the curated data was further investigated by using saliency maps \cite{kadir2001saliency}, which are visualizations of the gradient of model predictions with respect to their input.  Saliency maps  are usually used in computer vision tasks to show  the model's attention when making a particular decision. We adopted the same concept and utilized plain gradient to produce sailency maps on the input sequences of the LSTM network. Figure \ref{saliency} shows examples of sailency maps for both non-incident and incident model predictions on the validation set. The locations associated with top 20 largest gradient magnitude are represented by the red dots. They indicate where the model was focused  when making the corresponding decision. Based on the saliency maps of the incident model predictions, the model tended to pay more attention at the end of upstream and downstream speed where the speed drop happened and less on the relative speed difference. For non-incident model predictions, the model's attention was more uniformly distributed in terms of locations on sequences. The model tended to look at the overall behavior of the sequences, comparing the upstream and downstream speed to see whether  any significant separation was present. The decision-making process of the trained LSTM network largely aligned with human intuition of determining whether  an incident was present. Saliency maps supported understanding the trained model and the verification of the model correctness and usefulness. 




% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.7\linewidth]{images/saliency.png}
%     \caption{Examples of saliency maps of the LSTM network on the validation set. (a) shows the saliency maps on incident instances. The model's attention for predicting incident point lays largely at the end of upstream and downstream speed sequence (top row) and the place where the abrupt change happens (bottom row). (b) shows the saliency maps for non-incident predictions where the model's attention lays around the beginning of sequences (top row) and throughout (bottom row).}
%     \label{saliency}
% \end{figure}

\end{comment}

% The results contain the model evaluation of the time slice classification task as well as the detection performance before and after the single event grouping process. The raw loop detector data was noisy and contained missing values. Developing a useful data-driven incident detection model requires high quality training data. In this work, in addition to adopting recurrent neural network to classify time slices and establishing single event grouping, we emphasize the importance of curating data in a way that models can make the most use of. The results of model performance using datasets obtained from 3 different stages in Table 1 imply steady improvement as more advanced processing and cleaning steps were involved. The datasets in the first stage preserved the most raw form where the traffic profiles were in their original scale and missing measurements could exist. Every time series was merely filtered by the incident duration and speed different criteria. Models trained on datasets from this stages generally did not perform well, where the California algorithm, which used solely the occupancy information, only reached incident-class F1 score of 0.01, detection rate 0.004 before grouping and 0.06 after grouping. The SVM-KNN ensemble model, SVM with engeered features, and our LSTM classifier, utilizing the information from all three profiles, were able to achieve higher F1 scores on the testing set, although still resulting in relatively low detection rate and high false alarm rate. The second stage datasets contained the forward filled, smoothed and normalized traffic profiles through the processes mentioned in Section 2. Using the same model building and training procedures, the model time slice classification and incident detection performance was drastically improved on the testing set compared to using the datasets in stage 1. In particular, while the F1 score of all models had improvement, it increased 0.2 for the California algorithm. The post-grouping detection rate and false alarm rate have also been improved by more than 0.1 for all models. The datasets in the last stage differed from them in the previous stage by having the corrected human errors. Human errors here refer to the cases where the marked incident intervals did not align with the expected traffic profile change. This could be due to late report of the incident which could contribute to the noise in data-driven model training. Therefore, such human errors were corrected in the training sets in the final stage. The benefit of doing the correction reflected on the slightly higher time slice classification performance, pre- and post-grouping detection rate, and slightly lower false alarm rate. (\textcolor{red}{SVM KNN is showing lower dr and higher far-- why?}). The performance of models trained on datasets curated from three different stages suggested the importance of preparing informative high quality data for model training and that data-centric machine learning could lead to great improvement in model performance. 

% Among the incident cases presented in the testing set, the models naturally resulted in three types of defections--correctly detected, falsely detected, and missed. Fig \ref{examples} shows examples of such cases. In the correctly detected case, the entire or parts of detection area overlaps with the ground truth incident interval
% \textbf{correctly detected examples, misclassified examples, false alarm examples; also can report slice classification results in terms of confusion matrix and ROC curve}

% include typical cases of \textbf{missed cases} and \textbf{falsely detected incidents}.


% \begin{table*}[!tbhp]
%     \centering
%     \caption{Prior to smoothing}
%     \begin{tabular}{lcccc}
%     & \multicolumn{2}{c}{w/o. Grouping} &\multicolumn{2}{c}{w. Grouping}\\
%          &  DR & FAR & DR & FAR\\
%       \hline
%     California Algorithm & 0.004 & 0.33 & 0.06 & 0.12\\
    
%     SVM KNN ensemble \cite{xiao2019svm}  & 0.31 & 0.61 & 0.32 & 0.30\\
    
%     SVM w. engineered features \cite{lin2020automated} & 0.18 & 0.41 & 0.46 & 0.08\\
    
%     LSTM & 0.75 & 0.68 & 0.52 & 0.31\\
    
    
%     \end{tabular}
  
%     \label{tab:my_label}
% \end{table*}



% \begin{table*}[!tbhp]
%     \centering
%     \caption{With smoothing and normalization}
%     \begin{tabular}{lcccc}
%     & \multicolumn{2}{c}{w/o. Grouping} &\multicolumn{2}{c}{w. Grouping}\\
%          &  DR & FAR & DR & FAR\\
%       \hline
%     California Algorithm & 0.29 & 0.59 & 0.57 & 0.22\\
    
%     SVM KNN ensemble \cite{xiao2019svm}  & 0.38 & 0.62 & 0.90 & 0.11\\
    
%     SVM w. engineered features \cite{lin2020automated} & 0.19 & 0.47 & 0.53 &0.09\\
    
%     LSTM & 0.57 & 0.62 & 0.86 & 0.11\\
    
    
%     \end{tabular}
  
%     \label{tab:my_label}
% \end{table*}
%\begin{table}[]
%    \footnotesize
%    \centering
%    \caption{\textbf{Hand-picking curation}. Time slice classification model performance on the validation set before and after data curation}
%    \begin{tabular}{l|ccccccc}
%        \hline
%        \hline
%         & \multicolumn{3}{c}{Non-incident class} & \multicolumn{3}{c}{Incident class} &  \\
%         &  Precision & Recall & F1 & Precision & Recall & F1 & Accuracy \\
%         &\\
%         \textbf{Before Hand-picking} & \\
%         \hline
%         Random Forest & 0.61 & 0.94 & 0.74 & 0.87 & 0.40 & 0.55& 0.67\\
%         KNN SVM ensemble & 0.58 & 0.82 & 0.68 & 0.68 & 0.40 & 0.50 & 0.61\\
%         LSTM & 0.70 & 0.92 & 0.79 & 0.87 & 0.58 & 0.69 & 0.75\\
%         \hline
%         \vspace{2em}\\
%         
%         \textbf{After Hand-picking}& \\
%         \hline
%         Random Forest & 0.92 & 0.93 & 0.92 & 0.93 & 0.89 & 0.91 & 0.92\\
%         KNN SVM ensemble & 0.82 & 0.74 & 0.78 & 0.75 & 0.83 & 0.79 & 0.79\\
%         LSTM & 0.92 & 0.83 & 0.87 & 0.83 & 0.92 & 0.88 & 0.87\\
%         
%    \end{tabular}
%    
%    \label{cls_perf}
%\end{table}






\subsection{Incident detection}\label{detection}
\subsubsection{Metrics}

\begin{equation}
    DR = \frac{\text{Number of correctly detected incidents}}{\text{Number of total incidents}}
    \label{dr}
\end{equation}

\begin{equation}
    FAR = \frac{\text{Number of falsely detected incidents}}{\text{Number of detected incidents}}
    \label{far}
\end{equation}

%\PB{why this section is here; this should be moved to the experimental evaluation} \YS{moved}
The performance of a traffic incident detection model can be evaluated via two common metrics: detection rate  and false alarm rate. Detection rate represents the ratio of the number of correctly detected incidents to the number of ground truth incidents. It reflects the detection model's ability to capture potential characteristics of an incident.  The detection rate is  shown in Equation \ref{dr}. However, definitions of detection rate were not consistent in the literature. In \cite{el2018fuzzy} the numerator in the equation appeared to be the number of detected incidents. This is problematic because the number of detected incidents could potentially exceed the total number of incidents when the model makes many false detections. 

On the other hand, the false alarm rate is  the proportion of falsely detected incidents among all the detected incidents. The false alarm rate is defined in Equation \ref{far}. The inconsistency in the literature definitions also apply to FAR, where the number of non-incident cases was in the denominator  \cite{xiao2019svm, zhu2018deep}. This would lead to a low FAR since the number of non-incident cases is usually much larger than that of incidents. 

Therefore, we use the DR and FAR define in the Equations \ref{dr} and \ref{far} for the evaluation of the results in the rest of the our paper.

%We believe the following metrics are most reasonable for AID studies. The metric scores in the Results section were calculated according to Equations \ref{dr} and \ref{far} %\PB{You introduce 1 and 2 here but refer to them in the previous paragraph}.
%GAIL - I am not sure what "the following metrics"  and it seems awward to say the scores in the Results  section since you are  in the Results section unless  you mean the following subsubsection?


\subsubsection{Detection Results}
Here we present the incident detection results after applying the trained RNN with the  default LSTM cell and the deep ensemble model to the testing set. The original reported labels for the time slices in the testing set were noisy, with a considerable number of labels not matching the time slices' true behavior. Therefore, we report only the detection metric scores (DR, FAR) on 211 human-detectable incident cases from the testing set. The confirmation of when incidents happened was done visually. Our criterion was to look for incident indicators (speed drop, occupancy increase, and speed and occupancy separation) visually and compare them with the corresponding model detection results. DR and FAR were calculated based on the matches between the model detection and visual investigation. 
The model detection was based on the time slice classification results with two additional detection filters: (1) the time slices classified as incident with free-flow (normalized $>0.8$) speed on both upstream and downstream would be determined as non-incident since the traffic was not affected,  and (2) the number of consecutive time slices classified as incident had to exceed 6 steps (3 minutes) to be considered a detected incident. The LSTM network and deep ensemble model produced probability output for each instance in the testing set, and the final class labels were assigned based on the output threshold of 0.5 ( $>$ 0.5 incident class; $\leq$ 0.5 non-incident class). 

%\TM{do you mean -- incident class: probability output $>$ 0.5; non-incident class: probability output $<$ 0.5 }. 

The trained RNN with the default configurations made 231 incident detections, among which 203 were correctly detected and 28 were false alarms. It obtained a DR of 0.96 and an FAR of 0.12. The deep ensemble model was obtained after HPS for the default network and training using 50 different random seeds with the best configuration. Among the 50 models, 25 were selected based on their performance on the validation set (classification accuracy $>$ 0.9) to form the ensemble.  Given the uncertainty measure the deep ensemble model provided, we used a 75\% quantile of the probability outputs to assign labels. 

Figure \ref{detection} shows the detection examples from the deep ensemble model. The deep ensemble model was able to accurately detect the more obvious incidents, having low uncertainty at obvious regions (second plot in Figure \ref{detection}(a)), and it was improved by using the uncertainty measure. The use of the 75\% quantile of probability outputs improved detection on cases similar to the first plot in Figure \ref{detection}(b). However, the model tended to fail to detect incidents when the speed separation between the upstream and downstream was minor and when both speed profiles dropped abruptly but without any separation. 
%The usage of quantified uncertainty in this study was not to its extent. 
%It is worth investigating the information conveyed by regions with high uncertainty because
When the model failed to detect the incidents, it  usually had larger uncertainties. 

%While we did not leverage this to i 


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{images/detection_UQ.png}
    \caption{Detection results from the deep ensemble with a 75\% quantile of the probability outputs. The blue highlighted parts indicate detected incidents. (a) Examples with easy-to-detect incidents where the speed separation during incident was evident. (b) Harder examples---the first one demonstrates the advantage of using the 75\% quantile for classification where it successfully detected the incident while the mean values were not exceeding the threshold; the second plot implies that  incidents with minor speed separation might be hard for the model to detect; the third one shows the most easily missed cases where both the upstream and downstream speed had an abrupt drop while there was no speed separation.}
    \label{detection}
\end{figure}


Overall, the deep ensemble model with the 75\% quantile of probability output achieved 0.90 DR and 0.08 FAR with 168 correctly detected incidents and 12 false alarms. Compared with the RNN-based model with default configuration, the deep ensemble model had lower DR and  lower FAR. This result was expected from the model evaluation on the validation set, in which the deep ensemble model had higher precision and lower recall on the positive (incident) data points while keeping the overall classification accuracy the same.




\subsection{Implementing real-time detection}
Our testing process highly resembled real-time detection. The time slices with the speed profile history were fed to the model, the model classified these slices, and then detection was made based on additional criteria. We envision a similar process for the model to work in real time. These steps are described in more detail below.
\begin{itemize}
    \item Obtain one-hour average upstream and downstream speed difference during normal traffic. The one-hour window should be as close to the detection period as possible. This can be done via a moving average with a one-hour window excluding the contribution brought by incident-related profiles.
    \item Stream time slices with speed profile history; offset the upstream speed with the one-hour average difference; obtain relative speed difference.
    \item Feed processed data to the model; get model predictions with the incident or non-incident labels.
    \item Raise ``require attention" flag when the coming time slices are classified as incident slices.
    \item Raise ``incident detected" flag when there are more than 6 consecutive ``require attention" flags.
\end{itemize}

Figure \ref{realtime} shows the process of real-time detection. This process is robust to the possible noise present in the loop detector measurements. In particular, the ``require attention" status can act as a buffer for determining whether the classified incident slices are resulting from faulty measurements. Consequently, the detection is bound to be at least 6 steps (3 minutes) later than the actual starting time of the incidents.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/realtime.png}
    \caption{Real-time incident detection process using the deep ensemble model. (a)  Normal traffic -- model output probability is low with low uncertainty; (b) ``Require attention" status -- model output probability exceeded the threshold but the consecutive number of classified incident slices did not meet incident status; (c) Status changed to ``incident detected" after the number of consecutive classified incident slices went over 6; (d) Detection results for additional time.}
    \label{realtime}
\end{figure}


% \begin{table*}[!tbhp]
%     \centering
%     \caption{Detection rate and false  alarm rate scores of different AID models on the testing set.}
%     \begin{tabular}{lcccc}
%     & \multicolumn{2}{c}{w/o. Grouping} &\multicolumn{2}{c}{w. Grouping}\\
%          &  DR & FAR & DR & FAR\\
%       \hline
%     California Algorithm & 0.14 & 0.48 & 0.35 & 0.15\\
    
  
%      SVM KNN ensemble \cite{xiao2019svm}  & 0.38 & 0.59 & 0.90 & 0.09\\
    
%     SVM w. engineered features \cite{lin2020automated} & 0.22 & 0.49 & 0.56 & 0.12\\
    
%     LSTM & 0.65 & 0.47 & 0.81 & 0.12\\
    
    
%     \end{tabular}
  
%     \label{tab:my_label}
% \end{table*}


% \begin{table*}[h!]
%     \centering
%     \makebox[\textwidth]{\begin{tabular}{l*{15}{c}}
%          & \multicolumn{5}{c}{\textbf{Pre-smoothing}} & \multicolumn{5}{c}{\textbf{Post-smoothing}} & \multicolumn{5}{c}{\textbf{Correct Human Error}}\\
%          \hline
%          & & \multicolumn{2}{c}{w/o. Grouping} & \multicolumn{2}{c}{w.Grouping} & & \multicolumn{2}{c}{w/o. Grouping} & \multicolumn{2}{c}{w.Grouping} & & \multicolumn{2}{c}{w/o. Grouping} & \multicolumn{2}{c}{w.Grouping} \\
%          & F1 & DR & FAR & DR & FAR & F1 & DR & FAR & DR & FAR & F1 & DR & FAR & DR & FAR\\
%     California Algorithm & 0.01 & 0.004 & 0.33 & 0.06 & 0.12 & 0.23 & 0.15 & 0.50 & 0.39 & 0.15& 0.24 & 0.15 & 0.50 & 0.39 & 0.14\\
%     SVM KNN ensemble \cite{xiao2019svm} & 0.34 & 0.31 & 0.61 & 0.33 & 0.30 & 0.40 & 0.39 & 0.59 & 0.91 & 0.08 & 0.40 & 0.40 & 0.60 & 0.90 & 0.09\\
%     SVM w. engineered features \cite{lin2020automated} & 0.27 &0.18 & 0.41 & 0.46 & 0.08 & 0.28 & 0.20 & 0.47 & 0.53 & 0.09 & 0.31 & 0.22 & 0.48 & 0.58 & 0.11\\
%     LSTM & 0.45 & 0.79 & 0.68 & 0.60 & 0.28 & 0.46 & 0.81 & 0.68 & 0.73 & 0.08 & 0.46 & 0.81 & 0.67 & 0.79 & 0.06\\
    
%     \end{tabular}}
%     \caption{replace this with evaluation on the validation set}
%     \label{tab:my_label}
% \end{table*}






==> Traffic incident detection/5-rel.tex <==
Automatic incident detection on traffic networks has been a research topic for decades. Starting in the 1970s, algorithms were developed to detect potential incidents on the traffic  networks. These AID algorithms were  based mostly on the information provided by the inductive loop detectors embedded in the freeway pavement, from which traffic occupancy and volume profiles could be recorded. Accordingly, with the usage of occupancy, the California algorithm \cite{levin1979incident} and its variations were developed. With the installations of dual-loop detectors that can record traffic speed information, the detecting methods were expanded. In general, these algorithms can be categorized into pattern-based algorithms, catastrophe-based methods, and statistical methods \cite{martin2001incident}. With abundant data available from the traffic systems nowadays, data-driven methods, such as ML model-based AID frameworks, have been receiving increased attention.

%\subsubsection*{Data-driven traffic incident detection} 

Traffic data, regardless of the type, can be complicated and noisy because of sophisticated road layouts, human recording of incidents, and faulty sensors. Using ML models to achieve detection from the traffic data has shown great advantages thanks to their ability to learn complex mappings from data. In this section we discuss prior work on using ML models to conduct AID.  While some work has been done on estimating secondary crashes \cite{kitali_likelihood_2018, wang_modeling_2019, park_real-time_2018}, we mainly discuss the studies focusing  on the initial events. 

%\subsubsection{Network-level detection}

Several studies focused on detecting whether there is an incident or congestion on a network level, where the detection model takes in the information of the entire traffic network of interest and decides whether an incident is happening within the network without specifying its location. \cite{ma2015large} adopted an RNN combined with a restricted Boltzmann machine to detect network-wide congestion based on GPS data collected from taxis. \cite{zhu2018deep}  developed a CNN-based model to detect incidents in urban traffic networks, where the GIS information was adopted to match the measured traffic parameters and recorded incidents. \cite{liu2019traffic} developed a spatiotemporal graphical model called a spatiotemporal pattern network to predict traffic dynamics in large networks and detect incidents by calculating anomaly scores. \cite{basso_deep_2021} made use of the data from Automatic Vehicle Identification (AVI) gates and devices installed in vehicles, as well as loop detector measurements to detect incident with a CNN model.  In \cite{bao_spatiotemporal_2019},  a spatiotemporal convolutional long short-term memory network (STCL-Net) was used to  predict the city-wide traffic crash risk, where a mixed data sources were used, including crash data, Taxi GPS data, land use, population, and weather information. \cite{huang_highway_2020} transformed the loop detector measurement to heat maps with horizontal axis the time and vertical axis the traffic direction, and applied a CNN model to detect crashes.

%\subsubsection{Sensor/link-level detection}

As opposed to network-level detection, sensor-level detection emphasizes the usage of local information. \cite{jiang2010automated} developed an AID model where the real-time traffic data were compared with the traffic parameter estimation using a moving average, and then incidents were detected according to the difference. \cite{motamed2016developing} used an SVM  to classify  incident or non-incident instances given traffic speed, flow, and occupancy information. \cite{fouladgar2017scalable} utilized the traffic information on the nodes of interest and their neighbors to construct a spatiotemporal model using CNN and RNN to detect congestion. This work is easily scalable because only the information on a few neighbor nodes is needed. \cite{popescu2017automatic} incorporated vehicle-to-infrastructure communications with the traffic parameters from loop detectors to detect incidents based on distance and time of changing lanes. \cite{singh2018deep} used a stacked autoencoder to generate a high-level representation of traffic surveillance videos and adopted one-class SVM to detect potential traffic accidents. \cite{xiao2019svm} proposed an ensemble of k-nearest neighbors and SVM to classify instances with speed, flow, and occupancy information into incident or non-incident. \cite{yang2020expressway} used CNN and extreme gradient boosting to detect incidents in expressways with data from microwave detectors. \cite{jiang_long_2020} adopted data with different temporal resolution and used  an LSTM-based model to  detect traffic crashes.  \cite{mercader_automatic_2020} proposed to use isolation forest, an unsupervised anomaly detection approach, with bluetooth traffic monitoring data to achieve automatic incident detection.  \cite{parsa_real-time_2019} developed a real-time traffic accident detection model using SVM and probabilistic neural network, and the data imbalance and oversampling were also discussed.  \cite{parsa_toward_2020} adopted different data, e.g., demographic information, land use, and weather features, to detect traffic accident with extreme gradient boosting (XGBoost).  %\PB{what are the limitations of these methods and how our method is superior to these methods} -- \YS{addressed in the following paragraph}

Network-level detection models rely on the specific traffic network they have been trained on, which cannot be used for a different setting. Thus, we aim to develop a sensor-level detection model so that it has the potential of being deployed at different locations. However, the senor-level detection methods described above  required various types of data,  were evaluated on synthetic data, or did not provide any model prediction uncertainty measure. Also, data quality, which can play an essential role in training effective models, was not mentioned in the previous studies. Our work addresses these issues. Specifically, we adopt a data-centric approach to utilize real-world loop detector speed measurements, curate preprocessed data to create high-quality datasets, develop RNN-based classifiers, and create a deep ensemble model to quantify the model predictive uncertainty.
% \PB{you have to emphasize the data curation aspect as well} -- \YS{added above}


%\PB{the following paragraph should go to the experimental section (metrics that we use for the evaluation}


% \subsection{Imbalanced Learning}
% Due to the nature of incidents, the number of incident cases is much less than the normal cases. Training a supervised learning model on such data introduces a data imbalance issue, which causes learners to fail. Data imbalance refers to the situation where the number of instances in some class is much less than others. It is important to address this issue in the training stage, for models will normally over-classify the majority class due to its greater prior probability, miss-classifying the minority instances more often. There are mainly two ways of tackling data imbalance: data-level methods and algorithm-level methods. The objective of using data-level methods is to create a balanced dataset by over-sampling the minority class or under-sampling the majority class. There are many methods that can achieve under- or over-sampling. The simplest form is duplicating minority instances and discarding majority instances. Some studies \cite{mani2003knn, kubat1997addressing, barandela2004imbalanced} were done to address the overfitting issue introduced by duplicating and loss of information introduced by discarding. Currently, one of the most popular over-sampling techniques is Synthetic Minority Over-sampling Technique (SMOTE) \cite{chawla2002smote}, which, instead of duplicating existing instances, generates new instances similar to the existing ones along a line among k-nearest neighbors in the feature space. This method has been widely used to generate balanced datasets due to its ability of strengthening class boundaries to improve discrimination and reduce overfitting. Another way of dealing with data imbalance is to adjust the learning model without altering the training data distribution. The most straight forward way is to introduce new loss functions for training, where the penalty for miss-classifying minority class instances is higher. Many loss functions \cite{cui2019class, wang2016training, lin2017focal} are designed to take into account the importance of minority class instances, among which focal loss \cite{lin2017focal} was designed originally for object segmentation in computer vision. In this work, we took the algorithm-level approach to address the data imbalance problem in time slice classification, and focal loss was used as the loss function to train the LSTM classifier. 



==> Traffic incident detection/6-conc.tex <==


We presented a data-centric supervised learning workflow for  sensor level traffic incident detection. The training and validation data quality were ensured via preprocessing (exponential smoothing; oscillation check) and curation (input-label pair check; data selection; upstream speed offset). Demonstration with  three different classification models, including the proposed RNN-based network, showed that models trained on the carefully curated data had enormous classification performance improvement. In addition, the proposed RNN-based network (LSTM cell by default) was tuned through a hyperparameter search. The tuned model configurations were used for creating the deep ensemble model, which provides quantified predictive uncertainties. The detection results on 211 sensor detectable cases in the testzving set show that for both the default RNN model and the deep ensemble model we can achieve a high detection rate (0.96; 0.90) and low false alarm rate (0.12; 0.08). A real-time incident detection process using our RNN-based model was suggested, in which three detection statuses would be returned from the process.
% \PB{there is a big mess with RVV vs LSTM; pick one and use that consistently; it is super confusing} -- \YS{changed all to RNN based model only mention LSTM cells in the default setting}

We point out a few limitations of the current work and suggest future work to address these limitations. (1) The proposed incident detection method greatly depends on the traffic dynamics where the stop-and-go conditions in rush hours resemble incident behavior, resulting in false alarms. For future work, we plan to incorporate traffic wave models to reduce false detection further.
%1) The process of curating the training and validation data greatly relied on manual effort. We plan to adopt weak supervision combined with domain knowledge-guided labeling functions to automate the data creation process. This will significantly enlarge the high-quality training set, covering richer representations of the classes. 
(2) The uncertainty measure provided by the deep ensemble model was not fully exploited. Our future work will involve evaluating different statistics of the output probability values to classify instances and creating protocols for making decisions at the regions with high predictive uncertainties. (3) Only speed and occupancy information from the loop detector measurements was used. Besides other loop detector measurements,  many other data sources, such as surveillance video feed and vehicle GPS information,  can be helpful for detecting incidents. We aim to combine information from different sources to develop incident detection models for data fusion to further improve detection accuracy.




